Near-Optimal Algorithms for Minimax Optimization

This paper resolves a longstanding open question pertaining to the design of near-optimal first-order algorithms for smooth and strongly-convex-strongly-concave minimax problems. Current state-of-the-art first-order algorithms find an approximate Nash equilibrium using $\tilde{O}(\kappa_{\mathbf x}+\kappa_{\mathbf y})$ or $\tilde{O}(\min\{\kappa_{\mathbf x}\sqrt{\kappa_{\mathbf y}}, \sqrt{\kappa_{\mathbf x}}\kappa_{\mathbf y}\})$ gradient evaluations, where $\kappa_{\mathbf x}$ and $\kappa_{\mathbf y}$ are the condition numbers for the strong-convexity and strong-concavity assumptions. A gap still remains between these results and the best existing lower bound $\tilde{\Omega}(\sqrt{\kappa_{\mathbf x}\kappa_{\mathbf y}})$. This paper presents the first algorithm with $\tilde{O}(\sqrt{\kappa_{\mathbf x}\kappa_{\mathbf y}})$ gradient complexity, matching the lower bound up to logarithmic factors. Our algorithm is designed based on an accelerated proximal point method and an accelerated solver for minimax proximal steps. It can be easily extended to the settings of strongly-convex-concave, convex-concave, nonconvex-strongly-concave, and nonconvex-concave functions. This paper also presents algorithms that match or outperform all existing methods in these settings in terms of gradient complexity, up to logarithmic factors.

==> sec/algorithm.tex <==
%!TEX root = paper.tex
\section{The general iteration}\label{sec:iteration}
In this section, we propose and analyze two general iterations which form the basis of the algorithms we consider in this paper. These two general iterations require the input function $f$ which is $\ell$-smooth and $f(\x, \cdot)$ is strongly concave for all $\x \in \XCal$ with a condition number $\bar{\kappa} = \ell/\bar{\mu} > 0$. More specifically, the first general iteration $\hat{\x} = \GCal_1(f, \bar{\x}, \bar{\epsilon})$ solves the proximal minimax optimization problem given by
\begin{equation}\label{giter:update_first}
\min_{\x \in \XCal} \max_{\y \in \YCal} \ g(\x, \y) = f(\x, \y) + \ell\|\x - \bar{\x}\|^2.  
\end{equation}
It takes the function $f$, the point $\bar{\x}$ and the tolerance $\bar{\epsilon}$ as input and returns the new point $\hat{\x}$ such that 
\begin{equation}\label{giter:criterion_first}
\max_{\y \in \YCal} \ g(\hat{\x}, \y) \ \leq \ \min_{\x \in \XCal} \max_{\y \in \YCal} \ g(\x, \y) + \bar{\epsilon}. 
\end{equation} 
The second general iteration $\hat{\y} = \GCal_2(f, \tilde{\x}, \tilde{\epsilon})$ solves the maximization problem given by 
\begin{equation}\label{giter:update_second}
\max_{\y \in \YCal} \ f(\tilde{\x}, \y). 
\end{equation}
It takes the function $f$, the point $\tilde{\x}$ and the tolerance $\tilde{\epsilon}$ as input and returns the new point $\hat{\y}$ such that 
\begin{equation}\label{giter:criterion_second}
\max_{\y \in \YCal} \ f(\tilde{\x}, \y) \ \leq \ f(\tilde{\x}, \hat{\y}) + \tilde{\epsilon}. 
\end{equation} 
Each step of the first general iteration is the combination of two fixed-point iterations and one-step inexact Nesterov's accelerated projected gradient ascent while each step of the second general iteration is exactly one-step Nesterov's accelerated projected gradient ascent; see Algorithm~\ref{algorithm:giter-I} and~\ref{algorithm:giter-II}. 
\begin{algorithm}[!t]\small
\caption{$\hat{\x} = \GCal_1(f, \bar{\x}, \x_0, \bar{\epsilon})$}\label{algorithm:giter-I}
\begin{algorithmic}[1]
\STATE \textbf{Initialize:} $k=0$, $\y_0 \in \YCal$ and $\z_0 = \y_0$. 
\REPEAT
\STATE $\tilde{\x} = \x_0$. 
\REPEAT 
\STATE $\tilde{\x} \leftarrow \proj_\XCal(\bar{\x} - (1/2\ell)\gradx f(\tilde{\x}, \z_k))$.
\UNTIL{$\|\tilde{\x} - \proj_\XCal(\bar{\x} - (1/2\ell)\gradx f(\tilde{\x}, \z_k))\| \leq \min\{1, \frac{\bar{\epsilon}}{5971968
\bar{\kappa}^{9/2}\ell D}\}$ is satisfied.}
\STATE $\tilde{\x}_k = \tilde{\x}$. 
\STATE $\y_{k+1} = \proj_\YCal(\z_k + (1/4\ell)\grady f(\tilde{\x}_k, \z_k))$. 
\STATE $\z_{k+1} = \y_{k+1} + \frac{2\sqrt{\bar{\kappa}}-1}{2\sqrt{\bar{\kappa}}+1}(\y_{k+1} - \y_k)$. 
\STATE $\x = \x_0$. 
\REPEAT 
\STATE $\x \leftarrow \proj_\XCal(\bar{\x} - (1/2\ell)\gradx f(\x, \y_{k+1}))$
\UNTIL{$\|\x - \proj_\XCal(\bar{\x} - (1/2\ell)\gradx f(\x, \y_{k+1}))\| \leq \frac{\sqrt{\bar{\epsilon}/2\bar{\kappa}\ell}}{36\bar{\kappa}}$ is satisfied.} 
\STATE $\x_{k+1} = \x$. 
\STATE $k \leftarrow k+1$. 
\UNTIL{$\|\y_k - \proj_\YCal(\y_k + (1/4\ell)\grady f(\x_k, \y_k))\| \leq \frac{\sqrt{\bar{\epsilon}/2\bar{\kappa}\ell}}{48\bar{\kappa}}$ is satisfied.}
\STATE \textbf{Output:} $\hat{\x} = \x_k$. 
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[!t]\small
\caption{$\hat{\y} = \GCal_2(f, \tilde{\x}, \tilde{\epsilon})$}\label{algorithm:giter-II}
\begin{algorithmic}[1]
\STATE \textbf{Initialize:} $k=0$, $\y_0 \in \YCal$ and $\z_0 = \y_0$. 
\REPEAT
\STATE $\y_{k+1} = \proj_\YCal(\z_k + (1/\ell)\grady f(\tilde{\x}, \z_k))$. 
\STATE $\z_{k+1} = \y_{k+1} + \frac{\sqrt{\bar{\kappa}}-1}{\sqrt{\bar{\kappa}}+1}(\y_{k+1} - \y_k)$. 
\STATE $k \leftarrow k+1$. 
\UNTIL{$\|\y_k - \proj_\YCal(\y_k + (1/\ell)\grady f(\tilde{\x}, \y_k))\| \leq \frac{\sqrt{\tilde{\epsilon}/2\ell}}{\bar{\kappa}}$ is satisfied.}
\STATE \textbf{Output:} $\hat{\y} = \y_k$. 
\end{algorithmic}
\end{algorithm}
\subsection{Convergence results}
In this subsection, we present the convergence results of our general iterations (cf. Algorithm~\ref{algorithm:giter-I} and~\ref{algorithm:giter-II}) in strongly-concave and concave settings respectively. We first consider the strongly concave setting and make the following assumption.  
\begin{assumption}\label{Assumption:giter-strongly-concave} 
The function and constraint set pair, $\left(f: \br^{m+n} \rightarrow \br, \ \XCal \times \YCal \subseteq \br^{m+n} \right)$ satisfies
\begin{enumerate}
\item $f(\cdot, \cdot)$ is $\ell$-smooth and $f(\x, \cdot)$ is $\bar{\mu}$-strongly concave for all $\x \in \br^m$. 
\item $\XCal$ and $\YCal$ are both convex and $\YCal$ is further bounded with a diameter $D > 0$.
\end{enumerate}
\end{assumption}
We further define the important functions accordingly: 
\begin{equation*}
\begin{array}{ll}
\Phi_g(\cdot) \ = \ \max_{\y \in \YCal} \ g(\cdot, \y), & \qquad \y_g^*(\cdot) \ = \ \argmax_{\y \in \YCal} \ g(\cdot, \y), \\
\Psi_g(\cdot) \ = \ \min_{\x \in \XCal} \ g(\x, \cdot), & \qquad \x_g^*(\cdot) \ = \ \argmin_{\x \in \XCal} \ g(\x, \cdot). 
\end{array}
\end{equation*}
Note that the function $g$ is strongly convex-concave under Assumption~\ref{Assumption:giter-strongly-concave}. Therefore, the functions are not only well defined and unique but admit some special structure. We provide the complete information in the following structural lemma and defer the proof to Appendix~\ref{app:lemmas}. 
\begin{lemma}\label{Lemma:giter-structure}
Under Assumption~\ref{Assumption:giter-strongly-concave}, we have
\begin{enumerate}[(a)]
\item A point $\x_g^*(\z)$ is the fixed point of $T_\z(\cdot) = \proj_\XCal(\bar{\x} - (1/2\ell)\gradx f(\cdot, \z))$ for any given $\z \in \br^n$. 
\item An operator $T_\z(\cdot) = \proj_\XCal(\bar{\x} - (1/2\ell)\gradx f(\cdot, \z))$ is a $1/2$-contraction for any $\z \in \br^n$. 
\item A function $\y_g^*(\cdot)$ is $\bar{\kappa}$-Lipschitz.
\item A function $\Phi_g(\cdot)$ is $4\bar{\kappa}\ell$-smooth and $\ell$-strongly convex with $\nabla\Phi_g(\cdot) = \gradx g(\cdot, \y_g^*(\cdot))$. 
\item A function $\x_g^*(\cdot)$ is $3$-Lipschitz. 
\item A function $\Psi_g(\cdot)$ is $4\ell$-smooth and $\bar{\mu}$-strongly concave with $\nabla\Psi_g(\cdot) = \grady g(\x_g^*(\cdot), \cdot)$. 
\end{enumerate}
where $\bar{\kappa} = \ell/\bar{\mu}$ denotes the universal condition number of $f(\x, \cdot)$ for all $\x \in \XCal$. 
\end{lemma}
We first provide some intuitions on the convergence property of Algorithm~\ref{algorithm:giter-I} and~\ref{algorithm:giter-II}. 
\begin{enumerate}
\item Part (a) and (b) in Lemma~\ref{Lemma:giter-structure} imply that the gradient complexity of fixed-point iteration to return a point $\tilde{\x}$ such that $\|\tilde{\x} - \x_g^*(\y)\| = O(\bar{\epsilon})$ is bounded by $O(\log(1/\bar{\epsilon}))$. Part (f) in Lemma~\ref{Lemma:giter-structure} implies $\nabla\Psi_g(\cdot) = \grady g(\x_g^*(\cdot), \cdot)$. This together with the $\ell$-smoothness of $f$ implies that the output of fixed-point iteration $\tilde{\x}$ guarantees $\|\grady g(\x, \y) - \Psi_g(\y)\| = O(\bar{\epsilon})$. To this end, the scheme in Algorithm~\ref{algorithm:giter-I} can be interpreted as an inexact accelerated projected gradient ascent for solving problem $\max_{\y \in \YCal} \Psi_g(\y)$. Part (f) in Lemma~\ref{Lemma:giter-structure} also implies that $\Psi_g$ is $4\ell$-smooth and $\bar{\mu}$-strongly concave. Therefore, the gradient complexity of Algorithm~\ref{algorithm:giter-I} to return a point satisfying Eq.~\eqref{giter:criterion_first} is bounded by $O(\sqrt{\bar{\kappa}}\log(1/\bar{\epsilon}))$. 
\item The scheme in Algorithm~\ref{algorithm:giter-II} is an exact accelerated projected gradient ascent for solving problem $\max_{\y \in \YCal} f(\tilde{\x}, \y)$. This implies that the gradient complexity of Algorithm~\ref{algorithm:giter-II} to return a point satisfying Eq.~\eqref{giter:criterion_second} is bounded by $O(\sqrt{\bar{\kappa}}\log(1/\bar{\epsilon}))$. 
\end{enumerate}
Now we are ready to present the convergence results of Algorithm~\ref{algorithm:giter-I} and~\ref{algorithm:giter-II} under Assumption~\ref{Assumption:giter-strongly-concave}. For the ease of presentation, we define $D_\x = \|\x_0 - \x_g^*(\y_0)\| < +\infty$. 
\begin{proposition}\label{Prop:giter-first-sc}
Under Assumption~\ref{Assumption:giter-strongly-concave}, the point $\hat{\x} = \GCal_1(f, \bar{\x}, \x_0, \bar{\epsilon})$ must satisfy Eq.~\eqref{giter:criterion_first} and the gradient complexity is bounded by 
\begin{equation*}
O\left(\log\left(\frac{\bar{\kappa}^{9/2}\ell(D_\x^2 + D^2)}{\bar{\epsilon}}\right) + \sqrt{\bar{\kappa}}\log\left(\frac{\bar{\kappa}^{9/2}\ell(D_\x^2 + D^2)}{\bar{\epsilon}}\right)\log\left(\frac{\ell D^2}{\bar{\epsilon}}\right)\right). 
\end{equation*}
\end{proposition}
\begin{proposition}\label{Prop:giter-second-sc}
Under Assumption~\ref{Assumption:giter-strongly-concave}, the point $\hat{\y} = \GCal_2(f, \tilde{\x}, \tilde{\epsilon})$ must satisfy Eq.~\eqref{giter:criterion_second} and the gradient complexity is bounded by 
\begin{equation*}
O\left(1 + \sqrt{\bar{\kappa}}\log\left(\frac{\ell D^2}{\tilde{\epsilon}}\right)\right). 
\end{equation*}
\end{proposition}
Then we consider the strongly-convex-concave setting and make the following assumption. 
\begin{assumption}\label{Assumption:giter-concave} 
The function and constraint set pair, $\left(f: \br^{m+n} \rightarrow \br, \ \XCal \times \YCal \subseteq \br^{m+n} \right)$ satisfies
\begin{enumerate}
\item $f$ is $\ell$-smooth and $f(\x, \cdot)$ is concave for all $\x \in \br^m$. 
\item $\XCal$ and $\YCal$ are both convex and $\YCal$ is further bounded with a diameter $D > 0$.
\end{enumerate}
\end{assumption}
We introduce a new function $f_\eta(\x, \y) = f(\x, \y) - (\eta/2D^2)\|\y - \y_0\|^2$. If the function $f$ satisfies Assumption~\ref{Assumption:giter-concave}, it is clear that the function $f_\eta$ satisfies Assumption~\ref{Assumption:giter-strongly-concave} with $\bar{\mu} = \eta/D^2$. This implies that the function $f_\eta$ can be used as the input to Algorithm~\ref{algorithm:giter-I} and~\ref{algorithm:giter-II} with the theoretical guarantee as presented in Proposition~\ref{Prop:giter-first-sc} and Proposition~\ref{Prop:giter-second-sc} for the function $f_\eta$. 

If $\eta > 0$ is sufficiently small, i.e., $\eta = O(\epsilon)$, we can prove that the output of $\GCal_1$ and $\GCal_2$ with an input function $f_\eta$ still satisfy Eq.~\eqref{giter:criterion_first} and~\eqref{giter:criterion_second}. More specifically, let $\hat{\x} = \GCal_1(f_{\bar{\epsilon}}, \bar{\x}, \x_0, \bar{\epsilon}/2)$ and $\hat{\y} = \GCal_2(f_{\tilde{\epsilon}}, \tilde{\x}, \tilde{\epsilon}/2)$, we provide the theoretical guarantee in the following propositions. 
\begin{proposition}\label{Prop:giter-first}
Under Assumption~\ref{Assumption:giter-concave}, the point $\hat{\x} = \GCal_1(f_{\bar{\epsilon}}, \bar{\x}, \x_0, \bar{\epsilon}/2)$ must satisfy Eq.~\eqref{giter:criterion_first} and the gradient complexity is bounded by
\begin{equation*}
O\left(\log\left(\frac{\ell(D_\x^2 + D^2)}{\bar{\epsilon}}\right) + \sqrt{\frac{\ell D^2}{\bar{\epsilon}}}\log\left(\frac{\ell(D_\x^2 + D^2)}{\bar{\epsilon}}\right)\log\left(\frac{\ell D^2}{\bar{\epsilon}}\right)\right). 
\end{equation*}
\end{proposition}
\begin{proposition}\label{Prop:giter-second}
Under Assumption~\ref{Assumption:giter-concave}, the point $\hat{\y} = \GCal_2(f_{\tilde{\epsilon}}, \tilde{\x}, \tilde{\epsilon}/2)$ must satisfy Eq.~\eqref{giter:criterion_second} and the gradient complexity is bounded by 
\begin{equation*}
O\left(1 + \sqrt{\frac{\ell D^2}{\tilde{\epsilon}}}\log\left(\frac{\ell D^2}{\tilde{\epsilon}}\right)\right). 
\end{equation*}
\end{proposition}
The proof techniques are based on the modification of Nesterov's estimated sequence~\cite[Section~2.2.5]{Nesterov-2018-Lectures} and a simple reduction. We defer the proof of all propositions to the appendix.

==> sec/final_macros.tex <==
%!TEX root = EM_singular_models.tex

% PDF margin etc settings
\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-6cm}
\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-4cm}
\addtolength{\textheight}{-1.1\headheight}
\addtolength{\textheight}{-\headsep}
\addtolength{\textheight}{-\footskip}
\setlength{\oddsidemargin}{0.5cm}
\setlength{\evensidemargin}{0.5cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% MACROS HERE

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\fixedpointtheta}{\widehat\theta_\obs}

\newcommand{\cover}{N}
\newcommand{\kinit}{\nu}
\newcommand{\cdelta}{c_\threshold}
\newcommand{\dndelta}{\omega}
\newcommand{\kndelta}{\Upsilon}
\newcommand{\kndeltanew}{\Psi}
\newcommand{\radii}{\mathcal{R}}
\newcommand{\event}{\mathcal{E}}
\newcommand{\kevent}{\mathcal{D}}


% Observations, dimension etc.
\newcommand{\dims}{\ensuremath{d}}
\newcommand{\samples}{\ensuremath{n}}
\newcommand{\obs}{\samples}
\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\realdim}{\ensuremath{\real^\dims}}

\newcommand{\smallthreshold}{\epsilon}

% some mathcal notations
\newcommand{\order}[1]{\ensuremath{\mathcal{O}\parenth{#1}}}

% Basic statistics notation
\newcommand{\xstar}{\ensuremath{x^*}}
\newcommand{\xbar}{\ensuremath{\bar{x}}}
% True parameter
\newcommand{\thetastar}{\ensuremath{\theta^*}}
% Estimate one
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}
% Estimate two
\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}
\newcommand{\thetabar}{\ensuremath{\bar{\theta}}}
\newcommand{\yvec}{\ensuremath{y}}
\newcommand{\Xmat}{\ensuremath{X}}

% Distributions
\newcommand{\distribution}{P}
\newcommand{\density}{f}
\newcommand{\gaussiandensity}{\phi}
\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{Ber}}}

% Spaces
\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}


% Brackets Size
\newcommand{\brackets}[1]{\left[ #1 \right]}
\newcommand{\parenth}[1]{\left( #1 \right)}
\newcommand{\bigparenth}[1]{\big( #1 \big)}
\newcommand{\biggparenth}[1]{\bigg( #1 \bigg)}
\newcommand{\braces}[1]{\left\{ #1 \right \}}
\newcommand{\abss}[1]{\left| #1 \right |}
\newcommand{\angles}[1]{\left\langle #1 \right \rangle}
\newcommand{\tp}{^\top}

% Generic vectors and scalars
\newcommand{\myvec}{u} % for generic vector
\newcommand{\myvectwo}{v} % for generic vector
\newcommand{\mymat}{B}
\newcommand{\set}{{A}}
\newcommand{\scalar}{\alpha}
\newcommand{\tvscalar}{\epsilon}
\newcommand{\tailboundscalar}{t}
\newcommand{\term}{U}
\newcommand{\myVarone}{\alpha_X}
\newcommand{\myVartwo}{\alpha_Y}
\newcommand{\myCovmat}{\Sigma}
\newcommand{\xcord}[1]{x^{(#1)}}
\newcommand{\xcordpop}[1]{X^{(#1)}}
\newcommand{\ycordpop}[1]{Y^{(#1)}}
\newcommand{\myVarthree}{\ensuremath{U}}
\newcommand{\myVarfour}{\ensuremath{V}}
\newcommand{\myfuntwo}{\ensuremath{g}}
\newcommand{\numsteps}{t}
\newcommand{\totalnumsteps}{T}
\newcommand{\seqalpha}[1]{\alpha_{#1}}
\newcommand{\seqnu}[1]{\nu^{(#1)}}
\newcommand{\imax}{\ell_\smallthreshold}
\newcommand{\basis}{e}
\newcommand{\radem}{\varepsilon}
\newcommand{\Tone}{T\ensuremath{_{0}}}
\newcommand{\Ttwo}{T\ensuremath{_{2}}}
\newcommand{\contractPar}[1]{\ensuremath{\gamma\parenth{#1}}}



% EM updates
\newcommand{\hidden}{Z}
\newcommand{\qfun}[2]{Q(#1\vert#2)}
\newcommand{\variable}{\theta}
\newcommand{\weights}{w}
\newcommand{\myfun}{q}
\newcommand{\gradf}{\nabla \myfun}
\newcommand{\hessf}{\nabla^2 \myfun}
\newcommand{\iter}{t}
\newcommand{\mupdate}{M}
\newcommand{\mupdategeneral}{\ensuremath{M^{GN}}}




% EM contractions
\newcommand{\contractgene}{\ensuremath{\gamma^{GN}}}
\newcommand{\updateMat}{\ensuremath{\Gamma_{\theta}}}
\newcommand{\mymatTheta}{\ensuremath{B_{\theta}}}
\newcommand{\sech}{\text{sech}}

% Nhat's macros 
\newcommand{\Rspace}{\ensuremath{\mathbb{R}}}
\newcommand{\Ecal}{\ensuremath{\mathcal{E}}}
\newcommand{\Ncal}{\ensuremath{\mathcal{N}}}
\newcommand{\gradient}{\ensuremath{\nabla}}
\newcommand{\smallweight}{\ensuremath{\epsilon^{sw}}}
\newcommand{\smallnorm}{\ensuremath{\rho^{sw}}}
\newcommand{\ball}{\ensuremath{\mathbb{B}}}
\newcommand{\sphere}{\ensuremath{\mathbb{S}}}

\newcommand{\diam}{\ensuremath{\text{diam}}}
\newcommand{\upper}{\ensuremath{\bar{C}}}
\newcommand{\sample}{\ensuremath{\xi}}
\newcommand{\weight}{\ensuremath{\pi}}
\newcommand{\contracasym}{\ensuremath{\rho}}
\newcommand{\Fishermatrix}{\ensuremath{\mathcal{I}}}
\newcommand{\barcontracasym}{\ensuremath{\bar{\rho}}}


\newcommand{\TrueDensity}{\ensuremath{f}}
\newcommand{\FitDensity}{\ensuremath{f}_{\theta}}
\newcommand{\FitDensityfree}{\ensuremath{f}_{\pi, \theta}}
\newcommand{\FitDensitygen}{\ensuremath{f}_{\pi, \theta_{1}, \theta_{2}}}
\newcommand{\FitDensitymore}{\ensuremath{f}_{G}}
\newcommand{\normDensity}{\ensuremath{\phi}}
\newcommand{\mean}{\ensuremath{\theta}}
\newcommand{\sd}{\ensuremath{\sigma}}
\newcommand{\parFOS}{\ensuremath{\gamma}}
\newcommand{\funQ}{\ensuremath{Q}}
\newcommand{\updateM}{\ensuremath{M}}
\newcommand{\weightFun}{\ensuremath{w}}
\newcommand{\mydefn}{\ensuremath{:=}}

% Universal constants
\newcommand{\unicon}{c}
\newcommand{\uniconnew}{c'}
\newcommand{\uniconone}{c_1}
\newcommand{\unicontwo}{c_2}

% some parameters that you may define
\newcommand{\scparam}{m} % strong  convexity parameter
\newcommand{\smoothness}{L} % smoothness parameter
\newcommand{\step}{h}


%%%%%%%%% Distributions and Random variables %%%%%%%%%%%
\newcommand{\rvg}{\xi} % to denote the random variable g
\newcommand{\threshold}{\delta}


%%%%%%%%% Basic Terms like defn, etal, tmix, polylog %%%%%%%%%%%
\newcommand{\defn}{:=}
\newcommand{\rdefn}{=:}
\newcommand{\etal}{{et al.}}
\newcommand{\polylog}{\text{poly-log}}

% Some vector/matrix norms
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\left\| #1\right\|_{#2}}
\newcommand{\enorm}[1]{\vecnorm{#1}{2}} % euclidean norm
\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{fro}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}
%%% EM paper
\newcommand{\constrainnorm}[1]{\vecnorm{#1}{[k]}} % euclidean norm


% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}

% Kullback-Leibler
\newcommand{\kull}[2]{\ensuremath{D_{\text{KL}}(#1\; \| \; #2)}}

% Probability
\newcommand{\Exs}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}

%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}

% \DeclareMathOperator{\det}{det}
\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\floor}{floor}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\child}{child}
\DeclareMathOperator{\parent}{parent}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\toeplitz}{toeplitz}




\newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3's }#1}
\theoremstyle{named}
\newtheorem*{namedtheorem}{Lemma}

%%%%%%%
\theoremstyle{plain}

% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{conjecture}{Conjecture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
  \settoheight{\widebarargheight}{\ensuremath{#1}}%
  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
    \hspace{0.3\widebarargdepth}%
    \addtolength{\widebarargheight}{0.3ex}%
    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
  {#1}}



%%% New version of \caption puts things in smaller type, single-spaced
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
        \vskip 0.8ex
        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
        \dimen0=\hsize
        \advance\dimen0 by -3em
        \ifdim \wd\@tempboxa >\dimen0
                \hbox to \hsize{
                        \parindent 0em
                        \hfil
                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                                {\bf #1.} #2
                                %%\unhbox\@tempboxa
                                }
                        \hfil}
        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
        \fi
        }
\makeatother



%% COMMENTING commands

\long\def\comment#1{}
\definecolor{battleshipgrey}{rgb}{0.52, 0.52, 0.51}
\definecolor{darkgray}{rgb}{0.66, 0.66, 0.66}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
\definecolor{darkspringgreen}{rgb}{0.09, 0.45, 0.27}
\definecolor{dukeblue}{rgb}{0.0, 0.0, 0.61}
\definecolor{olivedrab7}{rgb}{0.24, 0.2, 0.12}
\definecolor{darkblue}{rgb}{0.0, 0.0, 0.55}
\definecolor{darkscarlet}{rgb}{0.34, 0.01, 0.1}
\definecolor{candyapplered}{rgb}{1.0, 0.03, 0.0}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\mjwcomment}[1]{{\bf{{\red{{MJW --- #1}}}}}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\highlight}[1]{\textcolor{applegreen}{#1}}

% comment lines
\newcommand{\genecomment}[1]{{\bf{{\blue{{TEAM --- #1}}}}}}
\newcommand{\rrdcomment}[1]{{\bf{{\blue{{RRD --- #1}}}}}}
\newcommand{\nhcomment}[1]{{\bf{{\blue{{NH --- #1}}}}}}
\newcommand{\kkcomment}[1]{{\bf{{\darkgreen{{KK --- #1}}}}}}


\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}


==> sec/results_nc.tex <==
%!TEX root = paper.tex
\section{Acceleration for nonconvex minimax problem}\label{sec:acceleration}
In this section, we propose the accelerated algorithms for nonconvex minimax problems. The pseudocode is presented in Algorithm~\ref{algorithm:nsc} and~\ref{algorithm:nc}.
\begin{algorithm}[!t]
\caption{\bf Accelerated algorithm for nonconvex-strongly-concave problem}\label{algorithm:nsc}
\begin{algorithmic}
\STATE \textbf{Input:} $\x_0 \in \br^m$ and the tolerance $\epsilon \in (0, 1)$. 
\STATE \textbf{Initialize:} $\bar{\epsilon} = \frac{\epsilon^2}{144\bar{\kappa}^2\ell}$. 
\FOR{$t = 0, 1, 2, \ldots, T$}
\STATE $\x_{t+1} = \GCal_1(f, \x_t, \x_0, \bar{\epsilon})$. 
\ENDFOR
\STATE Randomly pick up $\hat{\x}_T$ from $\{\x_t\}_{0 \leq t \leq T-1}$ at uniform. 
\STATE \textbf{Output:} $\hat{\x}_T$. 
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[!t]
\caption{\bf Accelerated algorithm for nonconvex-concave problem}\label{algorithm:nc}
\begin{algorithmic}
\STATE \textbf{Input:} $\x_0 \in \br^m$, $\y_0 \in \YCal$ and the tolerance $\epsilon \in (0, 1)$. 
\STATE \textbf{Initialize:} $\bar{\epsilon} = \frac{\epsilon^2}{48\ell}$. 
\FOR{$t = 0, 1, 2, \ldots, T$} 
\STATE $\x_{t+1} = \GCal_1(f_{\bar{\epsilon}}, \x_t, \x_0, \bar{\epsilon}/2)$. 
\ENDFOR
\STATE Randomly pick up $\hat{\x}_{T+1}$ from $\{\x_t\}_{1 \leq t \leq T+1}$ at uniform. 
\STATE \textbf{Output:} $\hat{\x}_{T+1}$. 
\end{algorithmic}
\end{algorithm}

\subsection{Convergence results}
In this subsection, we present the convergence results of our algorithms for solving nonconvex-strongly-concave and nonconvex-concave minimax problems. We first make the assumption for the nonconvex-strongly-concave setting as follows. 
\begin{assumption}\label{Assumption:nsc} 
The function and constraint set, $\left(f: \br^{m+n} \rightarrow \br, \ \XCal \times \YCal \subseteq \br^{m+n} \right)$ satisfies\footnote{For simplicity, we follow the setup in~\cite{Thekumparampil-2019-Efficient} and assume $\XCal = \br^m$. However, the similar results and analysis can be directly extended to the case when $\XCal \neq \br^m$ is a convex set.}
\begin{enumerate}
\item $f(\cdot, \cdot)$ is $\ell$-smooth and $f(\x, \cdot)$ is $\bar{\mu}$-strongly concave for all $\x \in \br^m$. 
\item $\XCal = \br^m$ and $\YCal$ is a convex and bounded set with a diameter $D > 0$.
\end{enumerate}
\end{assumption}
Even though $f(\cdot, \y)$ is not necessarily convex for each $\y \in \YCal$, $f(\x, \cdot)$ is strongly concave, which along with the boundedness of $\YCal$ allows for an efficient solution of $\max_{\y \in \YCal}f(\x, \cdot)$. We provide the information on the structure of the functions $\Phi$ and $\y^*$ (cf. Eq.~\eqref{Def:SCSC-Potential}) in the following lemma. 
\begin{lemma}\label{Lemma:nsc-structure}
Under Assumption~\ref{Assumption:nsc}, we have
\begin{enumerate}[(a)]
\item A function $\y^*(\cdot)$ is $\bar{\kappa}$-Lipschitz and a function $\Phi(\cdot)$ is $2\bar{\kappa}\ell$-smooth and $\grad\Phi(\cdot) = \gradx f(\cdot, \y^*(\cdot))$.
\end{enumerate}
where $\bar{\kappa} = \ell/\bar{\mu}$ denotes the universal condition number of $f(\x, \cdot)$ for all $\x \in \XCal$. 
\end{lemma}
Denote $\Delta_\Phi = \Phi(\x_0) - \min_{\x \in \br^m} \Phi(\x)$, we provide theoretical guarantees in the following theorem. 
\begin{theorem}\label{Theorem:nsc-main}
Under Assumption~\ref{Assumption:nsc}, the iteration complexity of Algorithm \ref{algorithm:nsc} to return an $\epsilon$-stationary point of $\Phi$ (cf. Definition~\ref{Def:NSC-Stationary}) is bounded by $O(\ell\Delta_\Phi\epsilon^{-2})$ and the total gradient complexity of Algorithm \ref{algorithm:nsc} is bounded by 
\begin{equation*}
O\left(\frac{\sqrt{\bar{\kappa}}\ell\Delta_\Phi}{\epsilon^2}\log\left(\frac{\bar{\kappa}^{11/2}\ell^2(D_\x^2 + D^2)}{\epsilon^2}\right)\log\left(\bar{\kappa}^2\ell^2D^2/\epsilon^2\right)\right). 
\end{equation*}
\end{theorem}
Then we proceed to the nonconvex-concave setting. 
\begin{assumption}\label{Assumption:nc}
The function and constraint set, $\left(f: \br^{m+n} \rightarrow \br, \ \XCal \times \YCal \subseteq \br^{m+n} \right)$ satisfies\samethanks
\begin{enumerate}
\item $f(\cdot, \cdot)$ is $\ell$-smooth and $f(\x, \cdot)$ is concave for all $\x \in \br^m$.
\item $\XCal = \br^m$ and $\YCal$ is a convex and bounded set with a diameter $D > 0$.
\end{enumerate}
\end{assumption}  
Note that $\Phi$ is not necessarily differentiable since $f(\x, \cdot)$ is merely concave for each $\x \in \br^m$. Fortunately, the smoothness assumption guarantees that $\Phi$ is $\ell$-weakly convex. 
\begin{lemma}\label{Lemma:nc-structure}
Under Assumption~\ref{Assumption:nc}, we have
\begin{enumerate}[(a)]
\item A set $\argmax_{\y \in \YCal} f(\x, \y)$ can contain multiple points for all $\x \in \br^m$.  
\item A function $\Phi(\cdot)$ is $\ell$-weakly convex and $\gradx f(\cdot, \z) \in \partial\Phi(\cdot)$ in which $\z \in \argmax_{\y \in \YCal} f(\cdot, \y)$. 
\item A function $\Phi_{1/2\ell}(\cdot)$ is $4\ell$-smooth and $\grad\Phi_{1/2\ell}(\cdot) = 2\ell(\cdot - \prox_{\Phi/2\ell}(\cdot))$.  
\end{enumerate}
\end{lemma}
Denote $\Delta_\Phi = \Phi(\x_0) - \min_{\x \in \br^m} \Phi(\x)$, we provide theoretical guarantee in the following theorem. 
\begin{theorem}\label{Theorem:nc-main}
Under Assumption~\ref{Assumption:nc}, the iteration complexity of Algorithm \ref{algorithm:nc} to return an $\epsilon$-stationary point of $\Phi$ (cf. Definition~\ref{Def:NC-Stationary}) is bounded by $O(\ell\Delta_\Phi\epsilon^{-2})$ and the gradient complexity of Algorithm \ref{algorithm:nc} is bounded by 
\begin{equation*}
O\left(\frac{\ell^2 D\Delta_\Phi}{\epsilon^3}\log\left(\frac{\ell^2(D_\x^2 + D^2)}{\epsilon^2}\right)\log\left(\frac{\ell D^2}{\epsilon^2}\right)\right). 
\end{equation*}
\end{theorem}

==> sec/results_sc.tex <==
%!TEX root = paper.tex
\begin{algorithm}[!t]
\caption{\bf Near-optimal algorithm for strongly convex-concave problems}\label{algorithm:scsc}
\begin{algorithmic}
\STATE \textbf{Input:} $\x_0 \in \XCal$ and the tolerance $\epsilon \in (0, 1)$.
\STATE \textbf{Initialize:} $\tilde{\x}_0 = \x_0$, $\bar{\epsilon} = \frac{\epsilon\ell}{576\kappa^{5/2}\bar{\kappa}^3}$ and $\tilde{\epsilon} = \frac{\epsilon\ell}{8\bar{\kappa}}$.    
\FOR{$t = 0, 1, 2, \ldots, T$}
\STATE $\x_{t+1} = \GCal_1(f, \tilde{\x}_t, \x_0, \bar{\epsilon})$. 
\STATE $\tilde{\x}_{t+1} = \x_{t+1} + \frac{2\sqrt{\kappa}-1}{2\sqrt{\kappa}+1}(\x_{t+1} - \x_t) + \frac{1}{2\sqrt{\kappa}+4\kappa}(\x_{t+1} - \tilde{\x}_t)$. 
\STATE $\y_{t+1} = \GCal_2(f, \x_{t+1}, \tilde{\epsilon})$. 
\ENDFOR
\STATE \textbf{Output:} $(\x_{T+1}, \y_{T+1})$. 
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[!t]
\caption{\bf Near-optimal algorithm for strongly-convex-concave problems}\label{algorithm:scc}
\begin{algorithmic}
\STATE \textbf{Input:} $\x_0 \in \XCal$, $\y_0 \in \YCal$ and the tolerance $\epsilon \in (0, 1)$.
\STATE \textbf{Initialize:} $\tilde{\x}_0 = \x_0$, $\bar{\epsilon} = \frac{\epsilon^4}{73328\kappa^{5/2}(\ell D^2)^3}\min\{\kappa^{-1}, \epsilon/\ell D^2\}$ and $\tilde{\epsilon} = \frac{\epsilon^2}{64\ell D^2}\min\{\kappa^{-1}, \epsilon/\ell D^2\}$.    
\FOR{$t = 0, 1, 2, \ldots, T$}
\STATE $\x_{t+1} = \GCal_1(f_\epsilon, \tilde{\x}_t, \x_0, \bar{\epsilon})$. 
\STATE $\tilde{\x}_{t+1} = \x_{t+1} + \frac{2\sqrt{2\kappa}-1}{2\sqrt{2\kappa}+1}(\x_{t+1} - \x_t) + \frac{1}{2\sqrt{2\kappa}+8\kappa}(\x_{t+1} - \tilde{\x}_t)$. 
\STATE $\y_{t+1} = \GCal_2(f_\epsilon, \x_{t+1}, \tilde{\epsilon})$. 
\ENDFOR
\STATE \textbf{Output:} $(\x_{T+1}, \y_{T+1})$. 
\end{algorithmic}
\end{algorithm}
\section{Near-optimal acceleration for strongly-convex minimax problem}\label{sec:near_optimal}
In this section, we propose the near-optimal algorithms for strongly-convex minimax problems; see Algorithm~\ref{algorithm:scsc} and~\ref{algorithm:scc}. Our algorithms achieve the near-optimal acceleration since it successfully incorporates the momentum update in minimization and maximization problems simultaneously. When $\YCal = \{\y_0\}$ is a singleton set, our algorithm recovers an extension of G{\"u}ler's accelerated proximal point algorithm for the strongly convex minimization problem $\min_{\x \in \XCal} f(\x, \y_0)$; when $\XCal = \{\x_0\}$ is a singleton set, our algorithm recovers Nesterov's accelerated projected gradient algorithm for the concave maximization problem $\max_{\y \in \YCal} f(\x_0, \y)$.

\subsection{Convergence results}
In this subsection, we present the convergence results of our algorithms for solving strongly convex-concave and strongly-convex-concave minimax problems.
\begin{assumption}\label{Assumption:scsc} 
The function and constraint set, $\left(f: \br^{m+n} \rightarrow \br, \ \XCal \times \YCal \subseteq \br^{m+n} \right)$ satisfies
\begin{enumerate}
\item $f(\cdot, \cdot)$ is $\ell$-smooth. 
\item $f(\cdot, \y)$ is $\mu$-strongly convex for all $\y \in \br^n$ and $f(\x, \cdot)$ is $\bar{\mu}$-strongly concave for all $\x \in \br^m$. 
\item $\XCal$ and $\YCal$ are both convex and $\YCal$ is further bounded with a diameter $D > 0$.
\end{enumerate}
\end{assumption}
The following structural lemma provides further information about $\Phi(\cdot) = \max_{\y \in \YCal} f(\cdot, \y)$ in the strongly convex-concave setting. 
\begin{lemma}\label{Lemma:scsc-structure}
Under Assumption~\ref{Assumption:scsc}, we have 
\begin{enumerate}[(a)]
\item A function $\y^*(\cdot)$ is $\bar{\kappa}$-Lipschitz. 
\item A function $\Phi(\cdot)$ is $2\bar{\kappa}\ell$-smooth and $\mu$-strongly convex with $\grad\Phi(\cdot) = \gradx f(\cdot, \y^*(\cdot))$. 
\item A function $\x^*(\cdot)$ is $\kappa$-Lipschitz. 
\item A function $\Psi(\cdot)$ is $2\kappa\ell$-smooth and $\bar{\mu}$-strongly convex with $\grad\Psi(\cdot) = \grady f(\x^*(\cdot), \cdot)$. 
\end{enumerate}
where $\kappa = \ell/\mu$ and $\bar{\kappa} = \ell/\bar{\mu}$ denote the universal condition numbers of $f(\cdot, \y)$ for all $\y \in \YCal$ and $f(\x, \cdot)$ for all $\x \in \XCal$ respectively.  
\end{lemma}
Since $f$ is strongly convex-concave, our target is to find an $\epsilon$-saddle point defined by the distance gap (cf. Definition~\ref{Def:SCSC-Saddle}) given only access to the gradient of $f$. Denote $\Delta_\x = \|\x_0 - \x^*\|$, we proceed to provide theoretical guarantees for our algorithm under the strongly convex-concave setting.  
\begin{theorem}\label{Theorem:scsc-main}
Under Assumption~\ref{Assumption:scsc}, the iteration complexity of Algorithm \ref{algorithm:scsc} to return an $\epsilon$-saddle point of $f$ (cf. Definition~\ref{Def:SCSC-Saddle}) is bounded by $O(\sqrt{\kappa}\log(\kappa\bar{\kappa}^3\Delta_\x^2/\epsilon))$ and the total gradient complexity of Algorithm \ref{algorithm:scsc} is bounded by
\begin{equation*}
O\left(\sqrt{\kappa\bar{\kappa}}\log\left(\frac{\kappa\bar{\kappa}^3\Delta_\x^2}{\epsilon}\right)\log\left(\frac{\kappa^{5/2}\bar{\kappa}^{15/2}(D_\x^2 + D^2)}{\epsilon}\right)\log\left(\frac{\kappa^{5/2}\bar{\kappa}^3D^2}{\epsilon}\right)\right). 
\end{equation*} 
\end{theorem} 
Then we consider the strongly-convex-concave setting and make the following assumption. 
\begin{assumption}\label{Assumption:scc}
The function and constraint set, $\left(f: \br^{m+n} \rightarrow \br, \ \XCal \times \YCal \subseteq \br^{m+n} \right)$ satisfies
\begin{enumerate}
\item $f(\cdot, \cdot)$ is $\ell$-smooth. 
\item $f(\cdot, \y)$ is $\mu$-strongly convex for all $\y \in \br^n$ and $f(\x, \cdot)$ is concave for all $\x \in \br^m$.
\item $\XCal$ and $\YCal$ are both convex and $\YCal$ is further bounded with a diameter $D > 0$.
\end{enumerate}
\end{assumption}  
Since $f$ is strongly-convex-concave, our target is to find an $\epsilon$-saddle point defined by the duality gap (cf. Definition~\ref{Def:SCC-Saddle}) given only access to the gradient of $f$. Denote $\Delta_\x = \|\x_0 - \x^*\|^2$, we proceed to provide theoretical guarantees for our algorithm under the strongly-convex-concave setting.  
\begin{theorem}\label{Theorem:scc-main}
Under Assumption~\ref{Assumption:scc}, the iteration complexity of Algorithm \ref{algorithm:scc} to return an $\epsilon$-saddle point of $f$ is bounded by $O(\sqrt{\kappa}\log(\sqrt{\kappa}\ell(D^2 + \Delta_\x^2)/\epsilon))$ and the total gradient complexity of Algorithm \ref{algorithm:scc} is
\begin{equation*}
O\left(\sqrt{\frac{\kappa\ell D^2}{\epsilon}}\log\left(\frac{\sqrt{\kappa}\ell(D^2 + \Delta_\x^2)}{\epsilon}\right)\log\left(\frac{\sqrt{\kappa} \ell (D_\x^2 + D^2)}{\epsilon}\right)\log\left(\frac{\kappa\ell D^2}{\epsilon}\right)\right). 
\end{equation*} 
\end{theorem}
We provide the detailed proof of Theorem~\ref{Theorem:scsc-main} and Theorem~\ref{Theorem:scc-main} in the next two subsections. 
